Variational Open-Domain Question Answering

Retrieval-augmented models have proven to be effective in natural language processing tasks, yet there remains a lack of research on their optimization using variational inference. We introduce the Variational Open-Domain (VOD) framework for end-to-end training and evaluation of retrieval-augmented models, focusing on open-domain question answering and language modelling. The VOD objective, a self-normalized estimate of the R\'enyi variational bound, approximates the task marginal likelihood and is evaluated under samples drawn from an auxiliary sampling distribution (cached retriever and/or approximate posterior). It remains tractable, even for retriever distributions defined on large corpora. We demonstrate VOD's versatility by training reader-retriever BERT-sized models on multiple-choice medical exam questions. On the MedMCQA dataset, we outperform the domain-tuned Med-PaLM by +5.3% despite using 2.500$\times$ fewer parameters. Our retrieval-augmented BioLinkBERT model scored 62.9% on the MedMCQA and 55.0% on the MedQA-USMLE. Last, we show the effectiveness of our learned retriever component in the context of medical semantic search.

==> archives/method.tex <==
\todo[inline]{Remove this (old version)}

We introduce a general probabilistic framework for the training, estimation and regularization of ODQA models following the reader-retriever approach.

\subsection{Likelihood and Gradient}

Let be a question $\rvq \in \Xset$ with a set of potential answers $\Aset \subset \Xset$ with a correct answer $\rva \in \Aset$. In ODQA, the task is to find the correct answer $\rva$ for the question $\rvq$ given a large corpus of $N$ documents $\Dset \defeq \{\rvd_1,\ldots,\rvd_N \} \subset \Xset$. We adopt the reader-retriever framework parameterized by a parameter $\theta$. The reader model $\pth(\rva | \rvd, \rvq)$ is parameterized by a parameter $\theta_A \subset \theta$ and a retriever model $\pth(\rvd | \rvq)$ parameterized by $\theta_B \subset \theta$. The marginal answer likelihood can be expressed using the joint density $\pth(\rva, \rvd | \rvq) = \pth(\rva | \rvd, \rvq)\ \pth(\rvd | \rvq)$ as:

\begin{equation}\label{eq:likelihood}
    \pth(\rva | \rvq) \defeq  \sum_{\rvd \in \Dset} \pth(\rva, \rvd | \rvq) \ .
\end{equation}

The gradient with regards to the parameter $\theta$ of the log marginal likelihood factorizes as:

\begin{equation}\label{eq:gradient}
    \nabla \log \pth(\rva | \rvq) =  \Ex_{\pth(\rvd | \rva, \rvq)} \left[ \nabla \log \pth(\rva, \rvd | \rvq) \right] \ .
\end{equation}

\subsection{Importance Sampling}

In practice, sampling from $\pth(\rvd | \rvq)$ might be intractable due to the potentially large size of the corpus $\Dset$. Importance sampling allows estimating the likelihood using samples from another distribution $\rphi(\rvd | \rvq)$ parameterized by $\phi$ such that $\rphi(\rvd | \rva, \rvq) > 0$ where $\pth(\rvd | \rvq) > 0$. The marginal answer likelihood can be estimated using samples from $\rphi$ and the importance weights $\wall(\rva, \rvd) \defeq \frac{\pth(\rva, \rvd | \rvq)}{\rphi(\rvd | \rva, \rvq)}$. The following equality holds:

\begin{equation}\label{eq:iw-likelihood}
    \pth(\rva | \rvq) = \Ex_{\rphi(\rvd | \rva, \rvq)} \left[ \wall(\rva, \rvd) \right] \ .
\end{equation}

The same treatment can be applied to the gradient of the marginal log-likelihood, which can be estimated as

\begin{equation}\label{eq:iw-gradient}
    \nabla \log \pth(\rva, \rvd | \rvq) = \Ex_{\rphi(\rvd | \rva, \rvq)} \left[  \widetilde{\wall}(\rva, \rvd) \ \nabla \log \pth(\rva, \rvd | \rvq) \right]
\end{equation}

where the normalized importance weights are defined as $\widetilde{\wall}(\rva, \rvd) \defeq \frac{\wall(\rva, \rvd) }{\Ex_{\rphi(\rvd' | \rvq)} \left[  \wall(\rva, \rvd') \right]}$.

\subsection{Regularization with Rényi Divergences}

The quality of the gradient depends on the quality of the posterior $\pth(\rvd | \rva, \rvq)$ (equation \ref{eq:gradient}), however the posterior might be uninformative at initialization, which might block the model in a sub-optimal section of the parameter space. To circumvent this failure mode, we relax the optimization objective such as to limit the effect of the posterior $\pth(\rvd | \rva, \rvq)$ on learning. We implement this using Rényi Divergence Variational Inference \citep{Li2016-ph, Lievin2020-cm}. Given $\alpha < 1$, we define the Rényi bound as:

\begin{equation}\label{eq:renyi-bound}
    \RVB_\alpha(\rva, \rvq) \defeq \frac{1}{1-\alpha} \log \Ex_{\rphi(\rvd | \rva, \rvq)} \left[ \wall^{1-\alpha}(\rva, \rvd)\right] 
\end{equation}

with gradient:

\begin{equation}\label{eq:renyi-gradient}
    \nabla \RVB_{\alpha}(\rva, \rvq) = \Ex_{\rphi(\rvd | \rva, \rvq)} \left[  \widetilde{\wall^{1-\alpha}}(\rva, \rvd) \ \nabla \log \pth(\rva, \rvd | \rvq) \right]
\end{equation}

where the normalized weights are defined as $\widetilde{\wall^{1-\alpha}}(\rva, \rvd) \defeq \frac{\wall^{1-\alpha}(\rva, \rvd) }{\Ex_{\rphi(\rvd' | \rva, \rvq)} \left[  \wall^{1-\alpha}(\rva, \rvd') \right]}$. 

The Rényi bound is a lower bound to the log-likelihood for $\alpha \geq 0$ and allows interpolating between two key objectives for $\alpha = 0$ and $\alpha = 1$, defined by continuity as $\RVB_{\alpha = 1}(\rva, \rvq) \defeq \lim_{\alpha \rightarrow 1}\RVB_{\alpha}(\rva, \rvq)$:
%
\begin{align*}
  \RVB_{\alpha \geq 0}(\rva, \rvq) \leq & \log \pth(\rva | \rvq) \\
  \RVB_{\alpha = 0}(\rva, \rvq) =& \log \pth(\rva | \rvq) \\
  \RVB_{\alpha = 1}(\rva, \rvq) =& \Ex_{\rphi(\rvd | \rva, \rvq)} \left[ 
   \log \pth(\rva | \rvd, \rvq) 
  \right]
  - \kl\left[ \rphi(\rvd | \rva, \rvq) || \pth(\rvd | \rvq) \right] \ .
\end{align*}

For $\alpha \rightarrow 1$, maximizing this objective corresponds to maximizing the reader probability proportionally to $\rphi$ and minimizing the KL divergence between the retriever $\pth(\rvd|\rvq)$ and the proposal $\rphi(\rvd|\rvq)$, whereas for $\alpha=0$, the probabilities of the reader and retriever models is increased for documents with high probability under $\pth(\rvd | \rva, \rvq)$. Given a uniform proposal $\rphi$, the parameter $\alpha$ introduces a way to control the trade-off between exploration and exploitation in learning ODQA models.

Furthermore, $\alpha$ induces a bias between variance and bias of the gradient estimator, as $\lim_{\alpha \rightarrow 1} \wall^{1-\alpha} = 1$, the effective sample size increases for $\alpha \rightarrow 1$, and consequently the variance of the gradient estimate decreases. Nonetheless, $\nabla \RVB_{\alpha}(\rva, \rvq)$ is unbiased only for $\alpha=0$ but the gradient for $\nabla \RVB_{\alpha > 0}(\rva, \rvq)$ remains relevant to the learning ODQA models, as long as the proposal $\rphi$ is relevant to the task.

\section{Tractable Estimation}

ODQA models are built from large pretrained language models which are used to index web-scaled collections of documents (e.g. whole Wikipedia). Therefore, computational efficiency is a key challenge in ODQA. We introduce a general definition of the retriever and proposal models that allows for tractable estimation of the likelihood ratio, we present a tractable implementation of the retriever model, an estimation method without replacement for greater computational efficiency and finally present likelihood and gradient estimates that are ready for implementation.

\subsection{Retriever likelihood ratio}

The parameterization of $\pth(\rvd | \rvq)$ and $\rphi(\rvd | \rva, \rvq)$ needs to be chosen carefully, so the importance weights $\wall$ can be evaluated at a reasonable cost. In the general setting, we parameterize the retriever and proposal models using score functions $\fth: \Xset^2 \rightarrow \Rset$ and $\fphi: \Xset^2 \rightarrow \Rset$:

\begin{equation}\label{eq:parameterization}
    \pth(\rvd | \rvq) \defeq \frac{\exp{\fth(\rvq, \rvd)}}{\sum_{\rvd' \in \Dset} \exp{\fth(\rvq, \rvd')}}, \qquad \rphi(\rvd | \rva, \rvq) \defeq \frac{\exp{\fphi(\rvq, \rvd)}}{\sum_{\rvd' \in \Dset} \exp{\fphi(\rvq, \rvd')}} \ .
\end{equation}

This allows estimating the ratio of the two models without evaluating the normalizing constants $\sum_{\rvd' \in \Dset} \exp{\fth(\rvq, \rvd')}$ and $\sum_{\rvd' \in \Dset} \exp{\fphi(\rvq, \rvd')}$. Using $\zeta(\rvd) \defeq \frac{\exp{\fth(\rvq, \rvd)}}{\exp{\rphi(\rvq, \rvd)}}$, the following equality holds:

\begin{equation}\label{eq:ratio}
\frac{\pth(\rvd | \rvq)}{\rphi(\rvd | \rva, \rvq)} = \frac{\zeta(\rvd)}{\Ex_{\rphi(\rvd | \rva, \rvq)}\left[ \zeta(\rvd)\right]}
\end{equation}

\subsection{Top-K approximation}

\todo[inline]{to be written}


\subsection{Retriever scoring function}

We define the similarity function $\fth$ using a pre-trained BERT model. We denote the $d : \Rset^d \times \Rset^d \rightarrow \Rset$ a vector level scoring function (dot product, cosine similarity or negative L2 norm). For a couple of contextualized representations $(\xb, \yb) \in (\Rset^{L_\xb \times d}) \times (\Rset^{L_\yb \times d})$ of respective lengths $L_\xb$ and $L_\yb$ and of vector size $d$, we define the scoring function $\fth$ using $\MaxSim$ operator \cite{Khattab2020-tn} and learned temperature parameter $\tau_\theta >0$: 

\begin{align}
    \fth(\xb, \yb) \defeq \frac{\tau_\theta^{-1}}{L_\xb} \sum_{i \in L_\xb} \max_{j \in L_\yb} d(\hth(\xb)_i, \hth(\yb)_j) \ .
\end{align}

The function $\hth$ defines BERT followed by a postition-wise linear layer \cite{Khattab2020-tn} : $\hth(\xb) \defeq \mathrm{Linear}_\theta(\bert_\theta(\xb))$, which yields contextualized representations based on the input text.

Alternatively, we can follow the approach popularized in \cite{Karpukhin2020-di} (DPR) by applying the vector-level metric $d$ to the output of BERT at the CLS token. Howerver, ColBERT allows to compare tokens directly, whereas DPR only allows comparison global text representations.

\subsection{Sampling without replacement with priority sampling}

The size of the document set $\Dset$ and the distribution $\rphi(\rvd | \rva, \rvq) \approx \pth(\rvd | \rvq)$ might be unbalanced; most of the probability mass of might be concentrated in a few documents. Therefore, a sampling scheme without replacement can be used to minimize the variance of a the gradient estimate (equation \ref{eq:gradient}).

Given a set of probabilities $p_1, \dots, p_N$ and a function with values $f_1, \dots, f_N$, priority sampling \cite{Duffield2007-rd} allows estimating the sum $\sum_{i=1}^N p_i f_i$ using a subset of $K < P$ elements. Priority sampling is unbiased \citep{Duffield2007-rd} and near optimal \citep{Szegedy_undated-wh}. The method has been popularized by \citep{Vieira2017-yd, Kool2019-qw, Kool2019-qp}.

Using priority keys $p_i / u_i, u_{i}$ with $\mathcal{U} = u_1, \ldots, u_{n} \stackrel{\text { iid }}{\sim} \mathrm{Uniform}(0,1]$, and setting $\tau$ to be the $K+1$-th largest key, we define the set $\Sset \defeq \{ i \in [1, N] \ |\ p_i / u_i > \tau \}$. Using $s_i := \max(p_i,\tau)$, we have:

\begin{align}
    \Ex_{p(u_1,\ldots,u_N)}\left[\sum_{i\in \Sset} s_i f_i\right] = \sum_{i=1}^N p_i f_i \ .
\end{align}

The proposal model $\fphi$ can be defined as a checkpoint of $\fth$, a $BM25$ score or a mixture of both.

\subsection{Estimation of the Rényi bound}

Using the above parameterization and priority sampling with probabilities $p_i = \rphi(\rvd_i | \rvq)$,  threshold ${\tau}$ and the set $\Sset \defeq \{ \rvd \in \Dset \ |\ p_i / u_i > \tau \}$, the Rényi bound can be estimated using:

\begin{align*}
    \RVB_\alpha(\rva, \rvq) \approx &
    %\frac{1}{1-\alpha} \log \sum_{\rvd \in \Sset} s(\rvd) \wall^{1-\alpha}(\rva, \rvd)  \approx 
    \frac{1}{1-\alpha} \log \sum_{\rvd \in \Sset} \tilde{s}(\rvd) \left( \frac{\zeta(\rvd) \pth(\rva| \rvd, \rvq)}{\sum_{\rvd' \in \Sset} \tilde{s}(\rvd') \zeta(\rvd')} \right)^{1-\alpha}
\end{align*}

with gradient:

\begin{align*}
     \nabla \RVB_{\alpha}(\rva, \rvq) \approx& 
     %\sum_{\rvd \in \Sset} s(\rvd) \widetilde{\wall^{1-\alpha}}(\rva, \rvd) \ \nabla \log \pth(\rva, \rvd | \rvq) \approx
     \sum_{\rvd \in \Sset} \frac{s(\rvd) \left( \zeta(\rvd) \pth(\rva | \rvd, \rvq) \right)^{1-\alpha}}{\sum_{\rvd' \in \Sset} s(\rvd') \left( \zeta(\rvd') \pth(\rva | \rvd', \rvq) \right)^{1-\alpha}} \nabla \log \pth(\rva, \rvd | \rvq)
\end{align*}

where we use the normalized weights $\tilde{s}(\rvd) \propto s(\rvd)$ for further variance reduction (classic IS trick).


Both estimates are biased because of the estimation of the numerators, however they both converge to $\RVB_\alpha(\rva, \rvq)$ and $\nabla \RVB_{\alpha}(\rva, \rvq)$ for $|\Sset| \rightarrow \infty$.

The term $\nabla \log \pth(\rva, \rvd | \rvq) = \nabla \log \pth(\rva | \rvd, \rvq) + \nabla  \log \pth(\rvd | \rvq)$ might be intractable due to the normalizing constant of $\pth(\rvd | \rvq)$. We use the following approximation:

\begin{equation}\label{eq:gradient-retriever}
    \nabla  \log \pth(\rvd | \rvq) \approx \nabla \fth(\rvq, \rvd) - \sum_{\rvd' \in \Sset} \frac{s(\rvd')\zeta(\rvd')}{\sum_{\rvd'' \in \Sset} s(\rvd'')\zeta(\rvd'')} \nabla \fth(\rvq, \rvd') \ . 
\end{equation}


\section{Application to Multiple Choice ODQA}


\subsection{Multiple choice likelihood}

In the multiple-choice setting, a vector of $M$ answer options $\rmA \defeq [\rva_1, \ldots, \rva_M]$ is given. We denote $\rva$ the correct option and assume $\rva \in \rmA$. We define the vector of $M$ queries as $\rmQ = [\rvq_1, \ldots, \rvq_M]$ with $\rvq_j \defeq [\rva_j ; \rvq]$ where $[\cdot ; \cdot]$ denotes the concatenation operator. We denote a vector of $M$ documents $\rmD = [\rvd_1, \ldots, \rvd_M]$ and the set of $M$ combinations of documents $\rvd \in \Dset$ as $\Dset^{(M)}$. The set $\Dset^{(M)}$ contains $N^{M}$ document vectors. Given the $\times$ denoting the cartesian product and of set $\Sset_j$ of priority samples for each option $j$, we define:

\begin{align*}
    \pth(\rmD | \rmQ) \defeq & \prod_{j=1}^{M} \pth(\rvd_j | \rvq_j) \\
    \rphi(\rmD | \rmQ) \defeq & \prod_{j=1}^{M} \rphi(\rvd_j | \rvq_j) \\
    \pth(\rmA, \rmD | \rmQ) \defeq & \pth(\rva | \rvd, \rvq) \pth(\rvd | \rvq) \\ 
    s(\rmD) \defeq& \prod_{j=1}^{M} s(\rvd_j) \\
    \zeta(\rmD) \defeq& \prod_{j=1}^{M} \zeta(\rvd_j) \\
    \Sset^{(M)} \defeq & \Sset_1 \times \ldots \times \Sset_M \ .
\end{align*}

The Renyi bound can be estimated with:


\begin{align*}
    \RVB_\alpha(\rmA, \rmQ) \approx &
    \frac{1}{1-\alpha} \log \sum_{\rmD \in \Sset^{(M)}} s(\rmD) \left( \frac{\zeta(\rmD) \pth(\rmA| \rmD, \rmQ)}{\sum_{\rmD' \in \Sset^{(M)}} s(\rmD') \zeta(\rmD')} \right)^{1-\alpha}\\
     \nabla \RVB_{\alpha}(\rmA, \rmQ) \approx& 
     \sum_{\rmD \in \Sset^{(M)}} \frac{s(\rmD) \left( \zeta(\rmD) \pth(\rmA | \rmD, \rmQ) \right)^{1-\alpha}}{\sum_{\rmD' \in \Sset^{(M)}} s(\rmD') \left( \zeta(\rmD') \pth(\rmA | \rmD', \rmQ) \right)^{1-\alpha}} \nabla \log \pth(\rmA, \rmD | \rmQ) \ .
\end{align*}

\todo[inline]{paper not updated beyond this point}


\subsection{Tricks}

\paragraph{Sharing documents across answer options}

At each estimation step of the likelihood and the gradient, a batch $\Bset \defeq \cup_{j=1}^M \Sset_j$ of documents is retrieved. Samples could be re-used across answer options, however this causes some problems for $\alpha \neq 0$, and requires sub-sampling $\Sset^{(M)}$.

\paragraph{Temperature parameterization}

We parameterize the temperature parameter $\tau_\theta$ with a learnable parameter $\kappa$ initialized to zero and with a static parameter $\kappa_0$ initialized based on the statistics of the first batch of data such that the scores are distributed with variance $\sigma_0^2 = 1e^{-2}$. We define $\tau_\theta$ and $\kappa_0$ as:

\begin{align}
    \tau_\theta &\defeq \exp{ \kappa - \kappa_0} \\
    \kappa_0 &\defeq  \log \sqrt{\Var[f_{\theta}]} - \log \sigma_0 \ .
\end{align}

This parameterization regularizes the learned model temperature $\tau$ towards the initial temperature $\tau_0$ when used in conjunction with weight decay.

\subsection{Answer Agnostic Retriever}

The multiple-choice retriever formulation allows learning a model $\fth([\rvq ; \rva], \rvd)$ that depends both on the question and the query. When using the retriever in a more general setting, the answer option is not known. Therefore, we use distillation such that to teach the model $\fth(\rvq, \rvd)$ to mimic the output of a pre-trained model $\rphi([\rvq ; \rva], \rvd)$ for which the correct answer $\rva$ is provided. 

We use model distillation, which we implemented by minimizing the following KL divergence.

\begin{align}
    L_{\mathrm{distill}} 
    &\defeq \kl\Big( 
        \rphi(\rvd | [\rva ; \rvq])
        \ ||\ 
        \pth(\rvd | \rvq)
    \Big)  \ .
\end{align}

==> sections/medqa-vs-medwiki.tex <==
\begin{table}[!h]
  \caption{Open Domain Question Answering accuracy on the MedQA dataset}
  \label{tab:odqa-medqa-vs-medwiki}
  \centering
  \begin{tabular}{ccccc}
    \toprule
    \multicolumn{2}{c}{Model} &   & \multicolumn{2}{c}{ Answering Accuracy (\%)}                \\
    Reader & Retriever & source   & US & TW \\
    \midrule
    $\varnothing$ & ES & \cite{Jin_undated-jo}  & -- & --    \\
    BERT & ES & \cite{Jin_undated-jo}  & -- & --    \\
    MoP & ES &\cite{Meng2021-dp} & -- & --    \\
    \midrule
    $\varnothing$ & ES & ours  & -- & --    \\
    BERT (concat) & ES & ours  & $39.5$ & $39.1$  \\
    BERT (stack) & ES & ours  & -- & --  \\
    \midrule
    BERT & $\varnothing$ & ours & -- & -- \\
    GPT-3 (prompting) & $\varnothing$ & ours & -- & -- \\
    \midrule
    DPR & DPR & ours & -- & --    \\
    Colbert & Colbert & ours & -- & --    \\
    BERT (stack) & BERT & ours & -- & --    \\
    BERT (stack) & Colbert & ours & -- & --    \\
    \bottomrule
  \end{tabular}
\end{table}

==> tables/corpora.tex <==
\begin{tabular}{lcc}
\toprule
\bf  & \bf MedWiki & \bf FindZebra \\
\midrule
\# articles  & 293.6k & 30.7k  \\
\# passages & 7,766.9k & 711.9k \\
% \shortstack[l]{\# tokens \\per passage} & 200 [200 -- 200] & 200 [200 -- 200]  \\
% \midrule
% \addlinespace[0.1cm]
% Source 
% & \multicolumn{1}{p{0.4\linewidth}}{ \small Wikipedia}
% & \multicolumn{1}{p{0.4\linewidth}}{ \small GARD, GeneReviews, Genetics Home Reference, OMIM, Orphanet, and Wikipedia} 
\bottomrule
\end{tabular}

==> tables/odqa-medmcqa-results.tex <==
\begin{tabular}{llll|rr}
    \toprule
    %\multicolumn{2}{c}{\bf Model}  & \multicolumn{2}{c}{\bf Answering Accuracy (\%)}                \\
    \bf Method & \bf Reader & \bf Retriever & \bf QA training set &  \bf{Valid.} & \bf{Test}\\
    \midrule
    % VOD-QA & BioLinkBERT (base) & bi-encoder & $\emptyset$ & MedMCQA & -- / -- \\
    % \cmark & BioLinkBERT (base) & bi-encoder  & bi-encoder  & MedMCQA & 53.3 & -- \\
    % \addlinespace[0.1cm]
    % VOD-QA & BioLinkBERT (base) & Cross attn. & $\emptyset$ & MedMCQA & -- / -- \\
    VOD & BioLinkBERT & BM25 & MedMCQA & 51.6 & 55.3 \\
    VOD & BioLinkBERT & BioLinkBERT  & MedMCQA & \bf 58.3 & \bf 62.9 \\
    % \cmark & BioLinkBERT (base) & Cross attn. & bi-encoder  & MedMCQA $\rightarrow$ USMLE &  56.5 & -- \\
    % \cmark & BioLinkBERT (base) & Cross attn. & bi-encoder  & USMLE & 34.5 & -- \\
    % VOD & BioLinkBERT & BioLinkBERT  & MedMCQA + USMLE & 57.6 & ... \\
    \midrule
    Uniform baseline & -- & -- & -- & 25.0 & 25.0 \\
    Disjoint\footnotemark[1]  & PubMedBERT & DPR  & MedMCQA & 43.0 & 47.0 \\
    Zero-shot prompting\footnotemark[2] & GPT-3 & -- & -- & 44.0 & --  \\
    Zero-shot prompting\footnotemark[2] & GPT-3  & BM25 & -- & 46.7 & -- \\
    Zero-shot CoT prompting\footnotemark[2]  & GPT-3 & BM25 & -- & 48.8 & -- \\
    \midrule
    Human (passing score)\footnotemark[2]  & -- & -- & -- & $\geq 50$ & $\geq 50$\\
    Human (merit candidate)\footnotemark[2]  & -- & -- & -- & $\geq 90$ & $\geq 90$ \\
    \bottomrule
     \addlinespace[0.1cm]
     \multicolumn{6}{l}{\small
     \textsuperscript{1}\citet{Pal2022-ph},~~\textsuperscript{2}\citet{Lievin2022-an}
     }

  \end{tabular}

==> tables/odqa-results-old.tex <==
\begin{tabular}{lllll|cc}
    \toprule
    %\multicolumn{2}{c}{\bf Model}  & \multicolumn{2}{c}{\bf Answering Accuracy (\%)}                \\
    \bf Method & \bf Backbone & \bf Reader & \bf Retriever & \bf Training set & \bf MedMCQA & \bf USMLE \\
    \midrule
    VODQA & BioLinkBERT (base) & DPR & DPR & MedMCQA & 53.33 / -- & 46.27 \\
    VODQA & BioLinkBERT (base) & DPR & DPR & USMLE & -- / -- & $\approx$44 \\
    VODQA & BioLinkBERT (base) & X & DPR & MedMCQA & -- / -- & -- \\
    VODQA & BioLinkBERT (base) & X & DPR & USMLE & -- / -- & $\approx$45  \\
    \midrule
    DrQA & PubMedBERT (base) & X & DPR & MedMCQA & 43 / 47 & -- \\
    DrQA & BioLinkBERT (base) & X & BM25 & USMLE & -- & 40.0 \\
    DrQA & BioLinkBERT (large) & X & BM25 & USMLE & -- & 44.6 \\
    \bottomrule
  \end{tabular}

==> tables/odqa-usmle-results.tex <==
\begin{tabular}{llll|rr}
    \toprule
    \bf Method & \bf Reader & \bf Retriever & \bf QA training set &  \bf Valid. & \bf Test \\
    \midrule
    % VOD & bi-encoder  & $\emptyset$ & USMLE & -- \\
    % VOD & bi-encoder  & bi-encoder  & USMLE & -- & $\approx$44 \\
    % VOD & bi-encoder  & bi-encoder  & MedMCQA & -- & -- \\
    % VOD & bi-encoder  & bi-encoder  & MedMCQA $\rightarrow$ USMLE & -- & $\approx$44 \\
    % \addlinespace[0.1cm]
    %VOD & Cross attn. & $\emptyset$ & USMLE & -- \\
    VOD  & BioLinkBERT & BM25 & USMLE & 41.0 & 40.4 \\
    VOD & BioLinkBERT & BioLinkBERT  & USMLE & 45.8 & 44.7 \\
    VOD & BioLinkBERT & BioLinkBERT  & MedMCQA &  47.2 & 46.8 \\
    VOD & BioLinkBERT & BioLinkBERT  & MedMCQA $\rightarrow$ USMLE &  \bf 53.6 & \bf 55.0 \\
    % VOD & BioLinkBERT & BioLinkBERT  & MedMCQA + USMLE & 53.2 & 54.8 \\
    \midrule
    Uniform baseline & -- & -- & -- & 25.0 & 25.0 \\
    Custom BM25\footnotemark[1]  & -- & BM25 & -- & 38.3 & 36.1 \\
    \addlinespace[0.1cm]
    Disjoint\footnotemark[2]  & PubMedBERT & BM25 & USMLE & -- & 38.1 \\
    Disjoint\footnotemark[3]  & BioLinkBERT & BM25 & USMLE & -- & 40.0 \\
    Disjoint\footnotemark[3]  & BioLinkBERT-L & BM25 & USMLE & -- & 44.6 \\
    \addlinespace[0.1cm]
    % QA-GNN\footnotemark[4] & SapBERT & GNN & USMLE & -- & 38.0 \\
    % GreaseLM\footnotemark[5] & -- & -- & USMLE & -- & --\\
    % \addlinespace[0.1cm]
    Zero-shot prompting\footnotemark[4] & GPT-3 & -- & -- & -- & 46.0  \\
    Zero-shot prompting\footnotemark[4] & GPT-3 & BM25 & -- & -- & 47.3 \\
    Zero-shot CoT prompting\footnotemark[4]  & GPT-3 & BM25 & -- &  -- & 53.1 \\
    \midrule
    Human (passing score)\footnotemark[4]  & -- & -- & -- & $\geq 60$ & $\geq 60$\\
    \bottomrule
    \addlinespace[0.1cm]
    \multicolumn{6}{l}{\small
        \textsuperscript{1}\citet{Jin2021-jo},
        ~~\textsuperscript{2}\citet{Gu2021-jn},
        ~~\textsuperscript{3}\citet{Yasunaga2022-gl},
        % ~~\textsuperscript{4}\citet{Yasunaga2021-iv},
        % ~~\textsuperscript{5}\citet{Zhang2022-yc},
        ~~\textsuperscript{4}\citet{Lievin2022-an}
    }
  \end{tabular}

==> tables/qa-datasets.tex <==
\begin{tabular}{lccc}
\toprule 
\bf  & \bf MedMCQA & \bf USMLE & \bf FZ Queries\\
\midrule
Answer type & multiple-choice & multiple-choice & CUI (UMLS) \\
\addlinespace[0.1cm]
\# questions (train/valid./test) & 182.8k / 4.2k / 6.1k & 10.2k / 1.3k / 1.3k &  -- / -- / 248 \\
\# tokens per question & 19 [4 -- 349] & 158 [13 -- 801] & 17 [8 -- 89] \\
\# tokens per answer option & 5 [3 -- 60] & 6.6 [3 -- 61] & --  \\
% \midrule
\addlinespace[0.1cm]
Source 
& \multicolumn{1}{p{0.22\linewidth}}{ \centering \small AIIMS and NEET PG entrance exams}
& \multicolumn{1}{p{0.22\linewidth}}{ \centering \small National Medical Board Examination (US)} 
& \multicolumn{1}{p{0.22\linewidth}}{ \centering \small search queries registered on FindZebra} 
\\
\bottomrule
\end{tabular}

==> tables/related-work-old.tex <==
\renewcommand{\arraystretch}{1.0} % Default value: 1
  \begin{tabular}{ll@{\hspace{-1em}}ccc}
    \toprule
    \bf Method & \bf Retriever training & \bf \shortstack{End-to-end\\retriever learning} & \bf  Variational & \bf \shortstack{Retriever \\ Support}    \\ 
    \midrule
    DPR\textsuperscript{1}& Supervised & \xmark & \xmark & --  \\
    ColBERT\textsuperscript{2} & Supervised & \xmark  & \xmark& -- \\
    Contriever\textsuperscript{3} & ICT (improved) & \xmark & \xmark & --   \\
    FiD\textsuperscript{4} & Frozen DPR dual-encoder & \xmark & \xmark & --  \\
    RETRO\textsuperscript{5} & Frozen BERT dual-encoder & \xmark & \xmark & --  \\
    \addlinespace[0.2cm]
    ORQA\textsuperscript{6} & ICT + MLL\textsuperscript{*} & (\cmark) & \xmark & top-$K$ doc. \\
    RAG\textsuperscript{7} & MLL\textsuperscript{*}  + frozen DPR doc. encoder & (\cmark) & \xmark  & top-$K$ doc. \\
    REALM\textsuperscript{8} & ICT + MLL\textsuperscript{*} & \cmark & \xmark & top-$K$ doc.  \\
    $\EMDR$\textsuperscript{9} & ICT + Expectation-Maximization  & \cmark & \xmark & top-$K$ doc. \\
    Hindsight\textsuperscript{9}  & ColBERT init. + ELBO + MLL\textsuperscript{*} & \cmark & \cmark & top-$K$ doc.   \\
    \midrule
    VOD & Rényi variational bound & \cmark & \cmark & top-$P$ doc.\textsuperscript{$\dagger$}\\
    \bottomrule
    \multicolumn{5}{l}{
    \small \textsuperscript{*}MLL: marginal likelihood,
    ~~\textsuperscript{$\dagger$} $K \leq P \leq N$ ( $K$:\# of documents in a batch, $N$: corpus size, $P$: chosen)
    }\\
    \multicolumn{5}{l}{
    \small \textsuperscript{1}~\citet{Karpukhin2020-di},
    \textsuperscript{2}~\citet{Khattab2021-xu},
    \textsuperscript{3}~\citet{Izacard2021-te},
    \textsuperscript{4}~\citet{Izacard2020-ui}
    }\\
    \multicolumn{5}{l}{
    \textsuperscript{5}~\citet{Borgeaud2021-td},
    \textsuperscript{6}~\citet{Lee2019-mr},
    \textsuperscript{7}~\citet{Lewis2020-cg},
    \textsuperscript{8}~\citet{Guu2020-la}
    }\\
    \multicolumn{5}{l}{
    \textsuperscript{9}~\citet{Sachan2021-vq},
    \textsuperscript{10}~\citet{Paranjape2021-dp}
    }
  \end{tabular}
